Taking gradients through experiments: LSTMs and memory proximal policy optimization for black-box quantum control

In this work we introduce the application of black-box quantum control as an interesting rein- forcement learning problem to the machine learning community. We analyze the structure of the reinforcement learning problems arising in quantum physics and argue that agents parameterized by long short-term memory (LSTM) networks trained via stochastic policy gradients yield a general method to solving them. In this context we introduce a variant of the proximal policy optimization (PPO) algorithm called the memory proximal policy optimization (MPPO) which is based on this analysis. We then show how it can be applied to specific learning tasks and present results of nu- merical experiments showing that our method achieves state-of-the-art results for several learning tasks in quantum control with discrete and continouous control parameters.

==> ground_states.tex <==
\subsection{Ground state transitions}
\label{ground_states}
Another scenario that was recently addressed in an anlysis of the characteristics of the optimization problem behind controlling systems out of equilibrium~\cite{bukov2017machine} is the transition between ground states of different Hamiltonians.
The considered class of Hamiltonians was thereby defined to be the class of Ising Hamiltonians given by
\begin{align*}
H(J,g,h) &= J \sum_{i=1}^{L-1} I^{\otimes i-1} \otimes \sigma_x \otimes \sigma_x \otimes I^{\otimes L-(i+1)} \\
&+ g \sum_{i=1}^{L} I^{\otimes i-1} \otimes \sigma_z \otimes I^{\otimes L - i} \\
&+ h \sum_{i=1}^{L} I^{\otimes i-1} \otimes \sigma_x \otimes I^{\otimes L - i}
\end{align*} 
where the $\sigma_{\{x,y,z\}}$ again denote the Pauli matrices and $L$ specifies the number of particles. 
In this setting we furthermore set $J=g=-1$, leaving $h$ as the only free parameter specifing the strength of the magnetic field represented by $\sigma_x$.
From a mathematical perspective, the ground state $\ket{E_{min}(h)}$ of a given Hamiltonian $H(h)$ is then defined as the eigenvector of $H(h)$ corresponding to its lowest eigenvalue.

In the considered scenario we now choose the initial and target states to be $\ket{\psi_i}=\ket{E_{min}(h_i)}$ and $\ket{\psi^*}=\ket{E_{min}(h^*)}$ respectively where $h_i \neq h^*$ are particular choices of $h$.
The controlled time evolution operator is then simply defined to be the one generated by $H(h)$ as given by
\[
U(h_t) = e^{-i \Delta t /h H(h_t)}
\]
where we assume $h_t$ to be time dependent.
The closeness between the state resulting from the controlled time evolution $\ket{\psi(T)}$ and the target state $\ket{\psi^*}$ is measured by their squared overlap
\[
S_2(\psi^*, \psi(T)) = |\braket{\psi^*, \psi(T)}|^2,
\]
similar to what was in Section~\ref{q_control}. 
We thus obtain the optimization problem formulation
\[
\max_{\{h_t\}} S_2(\psi^*, \psi(\{h_t\}))
\]

representing the quantum control scenario.


==> gs_rl.tex <==
%\section{Ground state transition as RL problem}

Next, we will introduce some RL tasks arising in this control scenario.
Similarly to the the taxonomy introduced above, we will thereby distinguish between a discrete, a continouous and a constrained case.
These cases correspond to different domains of possible values for the time dependent field strengths $h_t$. 
All of them however have in common that we assume a maximal magnitude $h_{max}$ of the field strength such that $h_t \in [-h_{max}, h_{max}]$ holds.
This is simply done to reflect the fact that in real experiments infinite field strengths are impossible to achieve.

\begin{description}
			\item[Discrete case] Knowing that the potentially continouous domain of our control parameter $h_t$ is upper and lower bounded by $\pm h_{max}$, we can apply Pontryagin's principle to limit ourselves to actions $s_t \in \{-h_{max}, h_{max}\}$. 
				We thus obtain a reinforcement learning problem where at each point in time the agent has to make a binary decision. 
				While this is arguably the easiest conceivable scenario, the sequence space still is of size $|S|=2^T$.

			\item[Continouous case] Although we know from theory that optimal sequences will comprise only extremal values of the control parameter $h_t$, it is still interesting to examine if the agent is able to discover this rule by itself.
				In this case we hence allow the agent to freely choose $h_t \in [-h_{max}, h_{max}]$ which again presents us with a sequence space of infinite size.
				Following our reasoning from the continouous quantum memory case, we cast the problem as learning the deviation $\Delta h \in [0, h_{max}]$ from $\pm h_{max}$.
				Hence, for each time $t$ the agent must predict the deviation $\Delta h$ and decide to which of the two extremal values the deviation should be applied.
				This formulation clearly allows the agent to predict any value in $[-h_{max}, h_{max}]$.

			\item[Constrained case] In the continouous case as defined above, we know that the agent should ideally learn to predict deviations of 0 to achieve sequences with extremal values of $h_t$.
					We can thus try to make the problem more challenging by imposing an upper bound $B < T|h_{max}|$ on $\sum_t |h_t|$, representing an upper limit of the total field strength.
					Imposing such a bound is not an artificial problem as it could for instance be used to model energy constraints in real experiments.
					This constraint can easily be realized by defining the reward of a sequence $s$ to be
					\[
					R(s) = 
					\begin{cases}
							S_2(\psi^*, \psi(s)) \; \text{if} \; \sum_t |h_t| \leq B \\
								0 \; \text{else}.
									
							\end{cases}
							\]
							This constraint requires the agent to learn how to distribute a global budget over a given sequence where it can maximally allocate an absolute field strength of $|h_{max}|$ to each action $s_t$.
							As it is not clear which values are optimal in principle for a given bound $B$, instead of a deviation we here let the agent directly predict the field strength $h_t$.


					\end{description}



==> qm_rl.tex <==
%\section{Quantum Memory as RL problem}
Having introduced the quantum memory scenario, we now turn to a description of possible reinforcement learning tasks in this context.
We present three different formulations of the setting which we will in the following refer to as the discrete, semi-continuous and continuous case. 
These formulations differ in the parametrization of the rotation $R_n(\alpha)$ that is to be performed at each time step.
\begin{description}
	\item[Discrete case] It is known from analytical derivations that the Pauli matrices $\sigma_{\{0, x,y,z\}}$ give rise to optimal sequences under certain ideal conditions~\cite{viola1999dynamical, souza2011robust}, where at each time step exactly one of the rotations $R_{\{0,x,y,z\}}=e^{-i \frac{\pi}{2} \sigma_{\{0,x,y,z\}}}$ is performed.
$\sigma_0$ hereby denotes the identity.
Hence, in the simplest formulation we can define the problem as chosing one of the four Pauli matrices at each time step.
This formulation then leads to a sequence space $S$ of size $|S|=4^T$ being exponential in the sequence length $T$.
This is the formulation which was also used in recent work on quantum memory~\cite{august2017using}.

\item[Semi-continuous case]
	While the class of sequences introduced above is provably ideal under certain conditions, one might be interested in allowing the agent more freedom to facilitate its adaption to more adverse conditions.
	This can in a first step be achieved by allowing the agent full control over the rotation angle while keeping the discrete formulation for the rotation axis.
	That means that at each time step, the agent will have to choose a rotation axis from $\sigma_{\{0,x,y,z\}}$ as before, but now must also predict the rotation angle $\alpha \in [0,2\pi]$.
	As $\alpha$ can take infinitely many values, this formulation of the problem now yields a sequence space $S$ of inifinite size, making it much harder from a reinforcement learning perspective.
	To lighten this burden we can make use of the fact that we know that in principle a rotation around $\pi$ is ideal.
	Thus, we will interpret the output of the agent as the deviation from $\pi$ $\Delta \alpha \in [-\pi, \pi]$.
	This should facilitate learning progress even in the early training phase.

	\item[Continuous case] Finally, we can of course also allow the agent full control over both the rotation angle and axis.
		This formulation of the problem requires the agent to predict a unit vector $n \in \mathbb{R}^3$ and a corresponding rotation angle $\alpha$ for each time step.
		It is clear that without any prior knowledge it will be very difficult for the agent to identify the `right corner' of this infinite sequence space.
		We hence propose to again leverage the knowledge about Pauli rotations being a good standard choice by having the agent predict a Pauli rotation together with the deviation in $n$ and $\alpha$.
		While for $\alpha$ we have already seen how this can be easily achieved, $n$ requires slightly more insight. 
		As is customary in quantum physics, every state of a two-dimensional particle $\ket{\psi}$ can be represented by choosing two angles $\theta \in [0,\pi]$ and $\phi \in [0, 2\pi]$, yielding the three-dimensional real unit Bloch vector
\[b =
\begin{pmatrix}
	\sin \theta \cos \phi \\
	\sin \theta \sin \phi \\
	\cos \theta
\end{pmatrix}.
\]
We can hence use this formulation to parameterize $n$ by $\theta$ and $\phi$. 
It is easy to see that the Pauli rotations correspond to the unit vectors that equal a one-hot encoding of the Pauli matrices such that we obtain the following identities
\begin{align*}
	\theta_x &= \theta_y = \phi_y = \frac{\pi}{2} \,\, \text{and} \\
	\phi_x &= \phi_z = \theta_z = 0
 \end{align*}
 with periodicity in $\pi$.
We can now leverage this knowledge by translating the Pauli rotation axis chosen by the agent into its Bloch expression and requring it to predict the deviations $\Delta \theta$ and $\Delta \phi$.
In this way the agent has access to the full axis space.
As with the rotation angle, this formulation has the effect that the agent starts learning from a reasonable baseline.
\end{description}


==> quantum_memory.tex <==
\section{Applying the Method}
In this section, we will now introduce two quantum control scenarios that were recently explored via machine learning~\cite{bukov2017machine, august2017using}. 
We show how one can apply our method to tackle some interesting learning tasks arising in these control settings by leveraging physical domain knowledge.

\subsection{Quantum Memory}
\label{quantum_memory}
One particular instance of a quantum control problem is the problem of storing the state of a qubit, i.e.\ a two-level system used in quantum computation. This is, next to quantum error correction, a very relevant problem in quantum computation.
Here we assume that our qubit is embedded in some environment, called the bath, such that the complete system lives in the Hilbert space
\begin{align*}
	\mathcal{H} = \mathcal{H}_S \otimes \mathcal{H}_B
\end{align*}
with the subsripts $S$ and $B$ denoting the space of the system and bath respectively. 
If we let this system evolve freely, decoherence effects will over time destroy the state of the qubit.
Hence the question is how we can intervene to prevent the loss of the state in the presence of the environment or, for computer scientific purposes, the noise where we assume to have control over the qubit only. From a quantum computing perspective, we would like to implement a gate that performs the identity function over a finite time interval.

Qubit states are commonly represented as points on the Bloch sphere~\cite{nielsen2002quantum} and the effect of the environment on the qubit can in this picture be perceived as some rotation that drives the qubit away from its original position.
To counter this problem we must hence determine a good rotation at each time step such that we negate the effect of the environment.
So, our goal is to dynamically decouple the qubit from its bath by performing these rotations.
The rotation of a qubit is defined as
\begin{align*}
	R_n(\alpha) = e^{-i\frac{\alpha}{2}n\mathbf{\sigma}}
\end{align*}
with $n$ being a unit vector specifying the rotation axis, $\alpha$ denoting the rotation angle and $\mathbf{\sigma}$ the `vector' of the stacked Pauli matrices $\sigma_{\{x,y,z\}}$~\cite{sakurai1995modern}.
Thus our controlled time evolution operator per time step $t$ becomes
\begin{align*}
	U(n_t, \alpha_t) = e^{-i \Delta t ( H_0 + \frac{\alpha_t }{2\Delta t}n_t\mathbf{\sigma} \otimes I_B)},
\end{align*}
expressing that we only apply the rotation to the qubit, but not the bath. 
The noise Hamiltonian $H_0$ here reflects the effect of the bath on the qubit and $I_B$ simply denotes the identity of size of the dimensionality of $\mathcal{H}_B$ such that the Kronecker product yields a matrix of equal size to $H_0$.

One possible metric to quantify how well we were able to preserve the qubit's state is
\begin{align*}
	D(U,I) = \sqrt{1 - \frac{1}{d_S d_B} \Vert \trace_S(U)\Vert_{\trace}}
\end{align*}
with $U$ denoting the total evolution operator, $I$ the identity and $\trace_S$ is the partial trace over the system~\cite{quiroz2013optimized}.
$\Vert U \Vert_{\trace} = \trace \sqrt{U^{\dagger}U}$ is the trace or nuclear norm.
This distance measure is minimized by the ideal case $U = I_S \otimes U_B$ with an arbitrary unitary $U_B$ acting on the bath.
Thus, the problem we would like to solve is a special instance of quantum control and can be formulated as
\begin{align*}
	\min_{\{(n_t, \alpha_t)\}} D(U(\{(n_t, \alpha_t)\}, I).
\end{align*}

